A Dependent Dependency Calculus (Extended Version)

Over twenty years ago, Abadi et al. established the Dependency Core Calculus (DCC) as a general purpose framework for analyzing dependency in typed programming languages. Since then, dependency analysis has shown many practical benefits to language design: its results can help users and compilers enforce security constraints, eliminate dead code, among other applications. In this work, we present a Dependent Dependency Calculus (DDC), which extends this general idea to the setting of a dependently-typed language. We use this calculus to track both run-time and compile-time irrelevance, enabling faster type-checking and program execution.

==> Sections/Heap.tex <==
\section{Flow-aware Semantics for DDC} \label{DDC-heap}
hhh


==> Sections/SDCC.tex <==
\section{Equivalence of SDC and DCC} \label{SDCC}

In this section, we show that SDC and the terminating fragment of DCC are equivalent. To this end, we first present a meaning-preserving translation from the terminating fragment of DCC to SDC. DCC programs are assigned meaning using a categorical model \textit{DC}. We shall also interpret SDC in the same model. But before that, we want to bring out an issue with the categorical model of DCC.

\subsection{An Issue with the Categorical Model of DCC}

The interpretation of DCC in category \textit{DC}, as presented in \citet{dcc}, is unsound. We explain the reason behind the unsoundness below. If we restrict ourselves to the terminating fragment of DCC, the objects of category \textbf{DC} are sets with label-indexed binary relations on them while the morphisms are functions that respect the relations. An object $C$ of category \textit{DC} is a set $| C |$ together with a family $R_{|C|,\ell}$ of binary relations on $| C |$ indexed by labels $\ell$. A morphism from $C$ to $D$ is a function $f$ from $| C |$ to $ D |$ such that for any $\ell$, if $ (c_1 , c_2) \in R_{| C |, \ell}$, then $( f c_1 , f c_2 ) \in R_{| D |, \ell}$.

The category is cartesian. The terminal object $\bd{1}$ is the singleton set with identity relation. Now, for objects $C, D$, the product $C \mathbf{\times} D$ is defined as:
\begin{align*}
| C \bd{\times} D | & = | C | \times | D | \\
R_{|C \bd{\times} D|, \ell} & = \{ ((c_1, d_1) , (c_2 , d_2)) \, | \, (c_1 , c_2) \in R_{|C|,\ell} \wedge (d_1 , d_2) \in R_{|D|,\ell} \}
\end{align*} 

But contrary to what is mentioned in \citet{dcc}, the category is not cartesian closed. In \citet{dcc}, the exponential object $D^C$, for objects $C, D$, has the set of morphisms from $C$ to $D$ as its underlying set. But this definition does not give us the required universal property for exponentials. We demonstrate this below.

Consider a two-point lattice $ { \color{black}{L} }   \leq   { \color{black}{H} } $. Consider objects $C , D, E$ such that 
\begin{align*}
| C | & = \{ c_1 , c_2 \} \\
| D | & = \{ d_1 , d_2 \} \\
| E | & = \{ e_1 , e_2 \} \\
R_{|C|, { \color{black}{L} } } & = | C | \times | C | \\
R_{|C|, { \color{black}{H} } } & = I_{|C|} \\
R_{|D|, { \color{black}{L} } } & = R_{|D|, { \color{black}{H} } } = I_{|D|} \\
R_{|E|, { \color{black}{L} } } & = R_{|E|, { \color{black}{H} } } = \{ (e_1 , e_1) \}
\end{align*} 
Here, $I_X$ represents the identity relation on $X$.

We can count that there are $8$ morphisms from $E \mathbf{\times} C$ to $D$ whereas there are only $2$ morphisms from $C$ to $D$. So $| D^C |$ has $2$ elements and thus, there can be at most $4$ morphisms from $E$ to $D^C$. Hence, $\textsf{Hom}(E \mathbf{\times} C , D)$ can not be isomorphic to $\textsf{Hom} (E , D^C)$. Therefore, the universal property of exponentials fails to hold. So the interpretation is unsound. 

If we analyse the problem, we find it stems from the fact that $(e_2 , e_2) \notin R_{| E |, \ell}$. Owing to this, a morphism can map $(e_2 , c_1)$ and $(e_2 , c_2)$ to unrelated values even though $c_1$ and $c_2$ are related. Generalizing this observation, we see that for any object $C$, the relation $R_{|C|,\ell}$ should be \textit{reflexive} for the interpretation to be sound. In fact, with this restriction, category \textit{DC} is a sound model of DCC. Henceforth, we refer to this restricted category as \textit{DC}.

Next, we interpret SDC in \textit{DC}.

\subsection{Categorical Model of SDC} 

Category \textit{DC} is a bicartesian closed category with a label-indexed monad $(\bd{T}^{\ell} , \bd{\eta}^{\ell} , \bd{\mu}^{\ell})$. The monad is defined as:
\begin{align*}
| \bd{T}^{\ell} (C) | & = | C | \\
R_{|\bd{T}^{\ell} (C)|, \ell_{{\mathrm{0}}}} & = R_{|C|, \ell} \text{ if } \ell  \leq  \ell_{{\mathrm{0}}} \text{ and } | C | \bd{\times} | C | \text{ otherwise} \\
\bd{T}^\ell (f : C \bd{\to} D) & = f \\
\bd{\eta}^{\ell}_C : C \bd{\to} \bd{T}^{\ell} (C) & = \bd{\lambda} x . x \\
\bd{\mu}^{\ell}_C : \bd{T}^\ell (\bd{T}^{\ell} (C)) \bd{\to} \bd{T}^{\ell} (C) & = \bd{\lambda} x . x 
\end{align*}
The cartesian product is described above. The coproduct $C \bd{+} D$ for objects $C, D$ is defined as:
\begin{align*}
| C \bd{+} D | & = | C | + | D | \\
R_{|C \bd{+} D|, \ell} & = \{ (\mathsf{inl } \, c_1 , \mathsf{inl } \, c_2) \, | \, (c_1 , c_2 ) \in R_{|C|,\ell} \} \cup \{ (\mathsf{inr } \, d_1 , \mathsf{inr } \, d_2) \, | \, (d_1 , d_2 ) \in R_{|D|,\ell} \}
\end{align*}
Lastly, the exponential $D^C$ for objects $C, D$ is given by:
\begin{align*}
| D^C | & = \mathsf{Hom} (C , D) \\
R_{| D^C |, \ell} & = \{ (f , g) \, | \, \forall (c_1 , c_2) \in R_{|C|,\ell} \Rightarrow (f c_1 , g c_2) \in R_{|D|,\ell} \}
\end{align*}

The following propositions hold in category \textit{DC}:
\begin{proposition}
\begin{enumerate}

\item $\bd{T}^{\ell} (C \bd{\times} D) = \bd{T}^{\ell} C \bd{\times} \bd{T}^{\ell} D$
\item $(\bd{T}^{\ell} D)^C = (\bd{T}^{\ell} D)^{\bd{T}^{\ell} C}$
\item $\bd{T}^{ \ell  \vee  \ell_{{\mathrm{0}}} } C = \bd{T}^{\ell} (\bd{T}^{\ell_{{\mathrm{0}}}} C)$
\item $\bd{T}^{ { \color{black}{\bot} } } C = C$
\item For $\ell_{{\mathrm{0}}}  \leq  \ell$, there exists a natural transformation $\tau^{\ell_{{\mathrm{0}}}  \leq  \ell}$ from $\bd{T}^{\ell_{{\mathrm{0}}}}$ to $\bd{T}^{\ell}$ such that for any object $C$, we have $\tau^{\ell_{{\mathrm{0}}}  \leq  \ell}_C = \bd{\lambda} x . x$. 
\end{enumerate}
\end{proposition}

But the following are \textbf{not} true in general: $\bd{T}^{\ell} (C \bd{+} D) = \bd{T}^{\ell} C \bd{+} \bd{T}^{\ell} D$ and $\bd{T}^{\ell} (D^C) = (\bd{T}^{\ell} D)^{\bd{T}^{\ell} C}$. With this understanding of the category, let us now look at the interpretation of SDC.

The types are interpreted as objects of the category:
\begin{align*}
  \llbracket  \ottkw{Unit}  \rrbracket  & = \bd{1} \\
  \llbracket   \ottnt{A}  \times  \ottnt{B}   \rrbracket  & =  \llbracket  \ottnt{A}  \rrbracket  \bd{\times}  \llbracket  \ottnt{B}  \rrbracket  \\
  \llbracket   \ottnt{A}  +  \ottnt{B}   \rrbracket  & =  \llbracket  \ottnt{A}  \rrbracket  \bd{+}  \llbracket  \ottnt{B}  \rrbracket  \\
  \llbracket   \ottnt{A}  \to  \ottnt{B}   \rrbracket  & =  \llbracket  \ottnt{B}  \rrbracket ^{ \llbracket  \ottnt{A}  \rrbracket } \\
  \llbracket   T^{ \ell }\;  \ottnt{A}   \rrbracket  & = \bd{T}^{\ell}  \llbracket  \ottnt{A}  \rrbracket 
\end{align*}

An open term $ \Omega  \vdash\,  \ottnt{b}  \, :^{ \ell }  \,  \ottnt{B} $ where $ \Omega = x_1 :^{\ell_{{\mathrm{1}}}} A_1 , x_2 :^{\ell_{{\mathrm{2}}}} A_2 , \ldots, x_n :^{\ell_{n}} A_n $ is interpreted as a morphism $ \llbracket  \ottnt{b}  \rrbracket  :  \llbracket  \Omega  \rrbracket  \bd{\to} \bd{T}^{\ell}  \llbracket  \ottnt{B}  \rrbracket $ where $ \llbracket  \Omega  \rrbracket  = \bd{T}^{\ell_{{\mathrm{1}}}}  \llbracket  \ottnt{A_{{\mathrm{1}}}}  \rrbracket  \bd{\times}  \bd{T}^{\ell_{{\mathrm{2}}}}  \llbracket  \ottnt{A_{{\mathrm{2}}}}  \rrbracket  \bd{\times} \ldots \bd{\times} \bd{T}^{\ell_n} \llbracket A_n \rrbracket$. With this interpretation, we show that category \textit{DC} is a sound model of SDC.

\begin{theorem}[Soundness] \label{soundness}
If $ \Omega  \vdash\,  \ottnt{a}  \, :^{ \ell }  \,  \ottnt{A} $, then $ \llbracket  \ottnt{a}  \rrbracket  \in \mathsf{Hom} ( \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell}  \llbracket  \ottnt{A}  \rrbracket )$.
\end{theorem}

\begin{proof}
By induction on $ \Omega  \vdash\,  \ottnt{a}  \, :^{ \ell }  \,  \ottnt{A} $.
\begin{itemize}
\item 
For \rref{SDC-Var}, we have $    \Omega_{{\mathrm{1}}} ,   \ottmv{x} \! :^{ \ell_{{\mathrm{0}}} }\! \ottnt{A}    ,  \Omega_{{\mathrm{2}}}   \vdash\,  \ottmv{x}  \, :^{ \ell }  \,  \ottnt{A} $ where $\ell_{{\mathrm{0}}}  \leq  \ell$. \\ Let $\Omega_{{\mathrm{1}}}$ be a list of length $k$. \\ Then $ \llbracket  \ottmv{x}  \rrbracket  \in \mathsf{Hom}( \llbracket  \Omega_{{\mathrm{1}}}  \rrbracket  \bd{\times} \bd{T}^{\ell_{{\mathrm{0}}}}  \llbracket  \ottnt{A}  \rrbracket  \bd{\times}  \llbracket  \Omega_{{\mathrm{2}}}  \rrbracket  , \bd{T}^{\ell}  \llbracket  \ottnt{A}  \rrbracket )$ is interpreted as: $ \llbracket  \ottmv{x}  \rrbracket  = \tau^{\ell_{{\mathrm{0}}}  \leq  \ell}_{ \llbracket  \ottnt{A}  \rrbracket } \circ \bd{\pi}_{k + 1}$.
\item
For \rref{SDC-Unit}, we have $ \Omega  \vdash\,  \ottkw{unit}  \, :^{ \ell }  \,  \ottkw{Unit} $. \\ Then $ \llbracket  \ottkw{unit}  \rrbracket $ is the unique morphism from $ \llbracket  \Omega  \rrbracket $ to $\bd{1}$.
\item
For \rref{SDC-Abs}, we have $ \Omega  \vdash\,   \lambda \ottmv{x} \!:\! \ottnt{A} . \ottnt{b}   \, :^{ \ell }  \,   \ottnt{A}  \to  \ottnt{B}  $ where $  \Omega ,   \ottmv{x} \! :^{  { \color{black}{\bot} }  }\! \ottnt{A}    \vdash\,  \ottnt{b}  \, :^{  { \color{black}{\bot} }  }  \,  \ottnt{B} $. \\ Using the inductive hypothesis, we get $  \llbracket  \ottnt{b}  \rrbracket  \in \textsf{Hom} (  \llbracket  \Omega  \rrbracket  \bd{\times}  \llbracket  \ottnt{A}  \rrbracket  ,  \llbracket  \ottnt{B}  \rrbracket )$. \\ Then, $ \llbracket   \lambda \ottmv{x} \!:\! \ottnt{A} . \ottnt{b}   \rrbracket  = \tau^{ { \color{black}{\bot} }   \leq  \ell}_{ \llbracket   \ottnt{A}  \to  \ottnt{B}   \rrbracket } \circ \textsf{curry}  \llbracket  \ottnt{b}  \rrbracket $.
\item
For \rref{SDC-App}, we have $ \Omega  \vdash\,   \ottnt{b}  \;  \ottnt{a}   \, :^{ \ell }  \,  \ottnt{B} $ where $ \Omega  \vdash\,  \ottnt{b}  \, :^{ \ell }  \,   \ottnt{A}  \to  \ottnt{B}  $ and $ \Omega  \vdash\,  \ottnt{a}  \, :^{  { \color{black}{\bot} }  }  \,  \ottnt{A} $. \\ Using the inductive hypothesis, we get, $ \llbracket  \ottnt{b}  \rrbracket  \in \mathsf{Hom} ( \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell} ( \llbracket  \ottnt{B}  \rrbracket ^{ \llbracket  \ottnt{A}  \rrbracket }))$ and $ \llbracket  \ottnt{a}  \rrbracket  \in \mathsf{Hom} ( \llbracket  \Omega  \rrbracket  ,  \llbracket  \ottnt{A}  \rrbracket )$. \\ Then, $ \llbracket   \ottnt{b}  \;  \ottnt{a}   \rrbracket  = \mathsf{app} \circ \langle  \llbracket  \ottnt{b}  \rrbracket  , \tau^{ { \color{black}{\bot} }   \leq  \ell}_{ \llbracket  \ottnt{A}  \rrbracket } \circ  \llbracket  \ottnt{a}  \rrbracket  \rangle$.
\item 
For \rref{SDC-Pair}, we have $ \Omega  \vdash\,   ( \ottnt{a}  ,  \ottnt{b} )   \, :^{ \ell }  \,   \ottnt{A}  \times  \ottnt{B}  $ where $ \Omega  \vdash\,  \ottnt{a}  \, :^{ \ell }  \,  \ottnt{A} $ and $ \Omega  \vdash\,  \ottnt{b}  \, :^{ \ell }  \,  \ottnt{B} $. \\ By inductive hypothesis, $ \llbracket  \ottnt{a}  \rrbracket  \in \mathsf{Hom} (  \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell}  \llbracket  \ottnt{A}  \rrbracket )$ and $ \llbracket  \ottnt{b}  \rrbracket  \in \mathsf{Hom} (  \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell}  \llbracket  \ottnt{B}  \rrbracket )$. \\ Then, $ \llbracket   ( \ottnt{a}  ,  \ottnt{b} )   \rrbracket  = \langle  \llbracket  \ottnt{a}  \rrbracket  ,  \llbracket  \ottnt{b}  \rrbracket  \rangle$.
\item 
For \rref{SDC-ProjF}, we have $ \Omega  \vdash\,   \pi_1\  \ottnt{a}   \, :^{ \ell }  \,  \ottnt{A_{{\mathrm{1}}}} $ where $ \Omega  \vdash\,  \ottnt{a}  \, :^{ \ell }  \,   \ottnt{A_{{\mathrm{1}}}}  \times  \ottnt{A_{{\mathrm{2}}}}  $. \\ By inductive hypothesis, $ \llbracket  \ottnt{a}  \rrbracket  \in \mathsf{Hom} (  \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell}  \llbracket   \ottnt{A_{{\mathrm{1}}}}  \times  \ottnt{A_{{\mathrm{2}}}}   \rrbracket )$. \\ Then $ \llbracket   \pi_1\  \ottnt{a}   \rrbracket  = \bd{\pi_1} \circ  \llbracket  \ottnt{a}  \rrbracket $. The \rref{SDC-ProjS} follows similarly.
\item 
For \rref{SDC-InjF}, we have $ \Omega  \vdash\,   \ottkw{inj}_1\,  \ottnt{a}   \, :^{ \ell }  \,   \ottnt{A}  +  \ottnt{B}  $ where $ \Omega  \vdash\,  \ottnt{a}  \, :^{ \ell }  \,  \ottnt{A} $. \\ By inductive hypothesis, $ \llbracket  \ottnt{a}  \rrbracket  \in \mathsf{Hom} ( \llbracket  \Omega  \rrbracket  ,  \llbracket  \ottnt{A}  \rrbracket )$. \\ Then $ \llbracket   \ottkw{inj}_1\,  \ottnt{a}   \rrbracket  = \tau^{ { \color{black}{\bot} }   \leq  \ell}_{ \llbracket   \ottnt{A}  +  \ottnt{B}   \rrbracket } \circ \bd{i_1}  \llbracket  \ottnt{a}  \rrbracket $. The \rref{SDC-InjS} follows similarly.
\item 
For \rref{SDC-Case}, we have $ \Omega  \vdash\,   \ottkw{case} \,  \ottnt{a} \, \ottkw{of}\,  \ottnt{b_{{\mathrm{1}}}}  ;  \ottnt{b_{{\mathrm{2}}}}   \, :^{ \ell }  \,  \ottnt{B} $ where $ \Omega  \vdash\,  \ottnt{a}  \, :^{ \ell }  \,   \ottnt{A_{{\mathrm{1}}}}  +  \ottnt{A_{{\mathrm{2}}}}  $ and $ \Omega  \vdash\,  \ottnt{b_{{\mathrm{1}}}}  \, :^{ \ell }  \,   \ottnt{A_{{\mathrm{1}}}}  \to  \ottnt{B}  $ and $ \Omega  \vdash\,  \ottnt{b_{{\mathrm{2}}}}  \, :^{ \ell }  \,   \ottnt{A_{{\mathrm{2}}}}  \to  \ottnt{B}  $. \\ By inductive hypothesis, $ \llbracket  \ottnt{a}  \rrbracket  \in \mathsf{Hom} ( \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell}  \llbracket   \ottnt{A_{{\mathrm{1}}}}  +  \ottnt{A_{{\mathrm{2}}}}   \rrbracket )$ and $ \llbracket  \ottnt{b_{{\mathrm{1}}}}  \rrbracket  \in \mathsf{Hom} ( \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell} ( \llbracket  \ottnt{B}  \rrbracket ^{ \llbracket  \ottnt{A_{{\mathrm{1}}}}  \rrbracket }))$ and $ \llbracket  \ottnt{b_{{\mathrm{2}}}}  \rrbracket  \in \mathsf{Hom} ( \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell} ( \llbracket  \ottnt{B}  \rrbracket ^{ \llbracket  \ottnt{A_{{\mathrm{2}}}}  \rrbracket }))$. \\ Then $ \llbracket   \ottkw{case} \,  \ottnt{a} \, \ottkw{of}\,  \ottnt{b_{{\mathrm{1}}}}  ;  \ottnt{b_{{\mathrm{2}}}}   \rrbracket  = \bd{T}^{\ell} (\mathsf{app}) \circ \langle \langle  \llbracket  \ottnt{b_{{\mathrm{1}}}}  \rrbracket  ,  \llbracket  \ottnt{b_{{\mathrm{2}}}}  \rrbracket  \rangle ,  \llbracket  \ottnt{a}  \rrbracket  \rangle$.
\item 
For \rref{SDC-Return}, we have $ \Omega  \vdash\,   \eta^{ \ell_{{\mathrm{0}}} }\;  \ottnt{a}   \, :^{ \ell }  \,   T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}  $ where $ \Omega  \vdash\,  \ottnt{a}  \, :^{  \ell  \vee  \ell_{{\mathrm{0}}}  }  \,  \ottnt{A} $. \\ By inductive hypothesis, $ \llbracket  \ottnt{a}  \rrbracket  \in \mathsf{Hom}( \llbracket  \Omega  \rrbracket  , \bd{T}^{ \ell  \vee  \ell_{{\mathrm{0}}} }  \llbracket  \ottnt{A}  \rrbracket )$. \\ Then, $ \llbracket   \eta^{ \ell_{{\mathrm{0}}} }\;  \ottnt{a}   \rrbracket  =  \llbracket  \ottnt{a}  \rrbracket $.
\item 
For \rref{SDC-Bind}, we have $ \Omega  \vdash\,   \ottkw{bind} ^{ \ell_{{\mathrm{0}}} } \,  \ottmv{x}  =  \ottnt{a}  \,  \ottkw{in}  \,  \ottnt{b}   \, :^{ \ell }  \,  \ottnt{B} $ where $ \Omega  \vdash\,  \ottnt{a}  \, :^{ \ell }  \,   T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}  $ and $  \Omega ,   \ottmv{x} \! :^{  \ell  \vee  \ell_{{\mathrm{0}}}  }\! \ottnt{A}    \vdash\,  \ottnt{b}  \, :^{ \ell }  \,  \ottnt{B} $. \\ By inductive hypothesis, $ \llbracket  \ottnt{a}  \rrbracket  \in  \mathsf{Hom}( \llbracket  \Omega  \rrbracket  , \bd{T}^{\ell} (\bd{T}^{\ell_{{\mathrm{0}}}}  \llbracket  \ottnt{A}  \rrbracket ))$ and $ \llbracket  \ottnt{b}  \rrbracket  \in \mathsf{Hom} ( \llbracket  \Omega  \rrbracket  \bd{\times} \bd{T}^{ \ell  \vee  \ell_{{\mathrm{0}}} }  \llbracket  \ottnt{A}  \rrbracket , \bd{T}^{\ell}  \llbracket  \ottnt{B}  \rrbracket )$. \\ Then $ \llbracket   \ottkw{bind} ^{ \ell_{{\mathrm{0}}} } \,  \ottmv{x}  =  \ottnt{a}  \,  \ottkw{in}  \,  \ottnt{b}   \rrbracket  =  \llbracket  \ottnt{b}  \rrbracket  \circ \langle \bd{id} ,  \llbracket  \ottnt{a}  \rrbracket  \rangle$.
\end{itemize}
\end{proof}

With this interpretation of SDC, we can relate it to DCC through category \textit{DC}.

\subsection{Meaning-preserving Translation of DCC into SDC}

In this section, we translate programs derived in the terminating fragment of DCC to programs in SDC such that the meaning of programs in category \textit{DC} is preserved. For this, we first translate DCC types to SDC types. We use $s , t$ for DCC types and $A, B$ for SDC types. Now, we define a function $\lceil \_ \rceil $ from DCC types to labels which gives us the maximum security clearance of a type.
\begin{align*}
\lceil \ottkw{Unit} \rceil & =  { \color{black}{\top} }  \\
\lceil \texttt{\textcolor{red}{<<no parses (char 7):  s -> t***  >>}} \rceil & = \lceil \ottnt{t} \rceil \\
\lceil \texttt{\textcolor{red}{<<no parses (char 10):  s times t***  >>}} \rceil & = \lceil \ottnt{s} \rceil \wedge \lceil \ottnt{t} \rceil \\
\lceil \texttt{\textcolor{red}{<<no parses (char 6):  s + t***  >>}} \rceil & =  { \color{black}{\bot} }  \\
\lceil \texttt{\textcolor{red}{<<no parses (char 8):  T psi s***  >>}} \rceil & = \ell \vee \lceil \ottnt{s} \rceil
\end{align*}

The maximum clearance function is closely related to the `protected at' judgement of \citet{dcc}. We recap this judgement in Figure \ref{fig:protected}. A type $\ottnt{s}$ is protected at a level $\ell$, written $\texttt{\textcolor{red}{<<no parses (char 10):  psi <<= s***  >>}}$, if $\ottnt{s}$ is allowed to see terms observable at $\ell$. We have the following relation between the protection judgement and the maximum clearance function.

\begin{figure}
\centering
\drules[Protect]{$\texttt{\textcolor{red}{<<no parses (char 10):  psi <<= s*** >>}}$}{}
{Unit,Fun,Prod,Sum,MonadE,MonadI}
\caption{Protection Judgement of DCC}
\label{fig:protected}
\end{figure}

\begin{lemma}
If $\texttt{\textcolor{red}{<<no parses (char 10):  psi <<= s***  >>}}$, then $\ell \leq \lceil \ottnt{s} \rceil$.
\end{lemma}
\begin{proof}
By induction on $\texttt{\textcolor{red}{<<no parses (char 10):  psi <<= s***  >>}}$.
\end{proof}
 
Now, we define the translation function ${}^{\overline{}}$ from DCC types to SDC types.
\begin{align*}
\texttt{\textcolor{red}{<<no parses (char 7):  D Unit*** >>}} & =  T^{  { \color{black}{\top} }  }\;  \ottkw{Unit}  \\
\texttt{\textcolor{red}{<<no parses (char 15):  D (\# s -> t \#)***  >>}} & = \texttt{\textcolor{red}{<<no parses (char 38):  T (\# M (\# s -> t \#) \#) ( D s -> D t )***  >>}} \\
\texttt{\textcolor{red}{<<no parses (char 18):  D (\# s times t \#)***  >>}} & = \texttt{\textcolor{red}{<<no parses (char 42):  T (\# M (\# s times t \#) \#) (D s times D t)***  >>}} \\
\texttt{\textcolor{red}{<<no parses (char 14):  D (\# s + t \#)***  >>}} & = \texttt{\textcolor{red}{<<no parses (char 34):  T (\# M (\# s + t \#) \#) (D s + D t)***  >>}} \\
\texttt{\textcolor{red}{<<no parses (char 16):  D (\# T psi s \#)***  >>}} & = \texttt{\textcolor{red}{<<no parses (char 46):  T (\# M (\# T psi s \#) \#) (\# T psi (\# D s \#) \#)***  >>}}
\end{align*} 

Note that the translation changes the type to one guarded by its maximum clearance. Since the initial type already had that clearance, the change is of a purely syntactic nature. In fact, we can show that both the types have the same meaning in category \textit{DC}.

\begin{lemma}
$ \llbracket   \overline{ \ottnt{s} }   \rrbracket  = \texttt{\textcolor{red}{<<no parses (char 8):  [\mbox{$\mid$} s \mbox{$\mid$}]***  >>}}$.
\end{lemma}

\begin{proof}
By induction on $s$.
\end{proof}

\begin{figure}
\centering
\drules[DCC]{$\texttt{\textcolor{red}{<<no parses (char 11):  G \mbox{$\mid$}- a : s***  >>}}$}{}
{Var,Unit,Lam,App,Pair,ProjF,ProjS,InjF,InjS,Case,Return,Bind}
\caption{DCC Type System}
\label{fig:dccType}
\end{figure}

Now, we translate open DCC terms to SDC terms. The DCC type system is presented in Figure \ref{fig:dccType}. Formally, given a DCC derivation $\texttt{\textcolor{red}{<<no parses (char 11):  G \mbox{$\mid$}- a : s***  >>}}$, we translate it to $\texttt{\textcolor{red}{<<no parses (char 26):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : D s***  >>}}$, where for $\Gamma =   \ottmv{x_{{\mathrm{1}}}}  :  \ottnt{s_{{\mathrm{1}}}}   ,   \ottmv{x_{{\mathrm{2}}}}  :  \ottnt{s_{{\mathrm{2}}}}  , \ldots, x_n : s_n$, we define $ \overline{ \Gamma }^{ \ell } $ as $  \ottmv{x_{{\mathrm{1}}}} \! :^{ \ell }\!  \overline{ \ottnt{s_{{\mathrm{1}}}} }   ,   \ottmv{x_{{\mathrm{2}}}} \! :^{ \ell }\!  \overline{ \ottnt{s_{{\mathrm{2}}}} }   , \ldots, x_n \! :^{\ell} \! \overline{s_n}$. For translating, we need some lemmas.

\begin{lemma}[Join] \label{join}
If $ \Omega  \vdash\,  \ottnt{a}  \, :^{ \ell }  \,   T^{ \ell_{{\mathrm{0}}} }\;  \ottsym{(}   T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}   \ottsym{)}  $, then there exists a term $ \ottkw{join}\,  \ottnt{a} $ such that $ \Omega  \vdash\,   \ottkw{join}\,  \ottnt{a}   \, :^{ \ell }  \,   T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}  $ and if $ \ottnt{a}  \leadsto  \ottnt{b} $, then $  \ottkw{join}\,  \ottnt{a}   \leadsto   \ottkw{join}\,  \ottnt{b}  $.
\end{lemma}

\begin{proof}
We have:
\begin{align*}
&   \Omega ,   \ottmv{x} \! :^{   \ell  \vee  \ell_{{\mathrm{0}}}   }\!  T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}     \vdash\,  \ottmv{x}  \, :^{  \ell  \vee  \ell_{{\mathrm{0}}}  }  \,   T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}   & \text{[By \rref{SDC-Var}]} \\
&     \Omega ,   \ottmv{x} \! :^{   \ell  \vee  \ell_{{\mathrm{0}}}   }\!  T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}     ,   \ottmv{y} \! :^{   \ell  \vee  \ell_{{\mathrm{0}}}   }\! \ottnt{A}    \vdash\,  \ottmv{y}  \, :^{   \ell  \vee  \ell_{{\mathrm{0}}}   }  \,  \ottnt{A}  &  \text{[By \rref{SDC-Var}]} \\ 
&   \Omega ,   \ottmv{x} \! :^{   \ell  \vee  \ell_{{\mathrm{0}}}   }\!  T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}     \vdash\,   \ottkw{bind} ^{ \ell_{{\mathrm{0}}} } \,  \ottmv{y}  =  \ottmv{x}  \,  \ottkw{in}  \,  \ottmv{y}   \, :^{  \ell  \vee  \ell_{{\mathrm{0}}}  }  \,  \ottnt{A}  & \text{[By \rref{SDC-Bind}]} \\
&   \Omega ,   \ottmv{x} \! :^{   \ell  \vee  \ell_{{\mathrm{0}}}   }\!  T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}     \vdash\,   \eta^{ \ell_{{\mathrm{0}}} }\;  \ottsym{(}   \ottkw{bind} ^{ \ell_{{\mathrm{0}}} } \,  \ottmv{y}  =  \ottmv{x}  \,  \ottkw{in}  \,  \ottmv{y}   \ottsym{)}   \, :^{ \ell }  \,   T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}   & \text{[By \rref{SDC-Return}]} \\
&  \Omega  \vdash\,   \ottkw{bind} ^{ \ell_{{\mathrm{0}}} } \,  \ottmv{x}  =  \ottnt{a}  \,  \ottkw{in}  \,   \eta^{ \ell_{{\mathrm{0}}} }\;  \ottsym{(}   \ottkw{bind} ^{ \ell_{{\mathrm{0}}} } \,  \ottmv{y}  =  \ottmv{x}  \,  \ottkw{in}  \,  \ottmv{y}   \ottsym{)}    \, :^{ \ell }  \,   T^{ \ell_{{\mathrm{0}}} }\;  \ottnt{A}   &  \text{[By \rref{SDC-Bind}]}
\end{align*}
Then, $ \ottkw{join}\,  \ottnt{a}  =  \ottkw{bind} ^{ \ell_{{\mathrm{0}}} } \,  \ottmv{x}  =  \ottnt{a}  \,  \ottkw{in}  \,   \eta^{ \ell_{{\mathrm{0}}} }\;  \ottsym{(}   \ottkw{bind} ^{ \ell_{{\mathrm{0}}} } \,  \ottmv{y}  =  \ottmv{x}  \,  \ottkw{in}  \,  \ottmv{y}   \ottsym{)}  $. Note that if $ \ottnt{a}  \leadsto  \ottnt{b} $, then $  \ottkw{join}\,  \ottnt{a}   \leadsto   \ottkw{join}\,  \ottnt{b}  $.
\end{proof}

\begin{theorem}[Forward Translation]
If $\texttt{\textcolor{red}{<<no parses (char 11):  G \mbox{$\mid$}- a : s***  >>}}$, then there exists $\texttt{\textcolor{red}{<<no parses (char 4):  D a***  >>}}$ such that $\texttt{\textcolor{red}{<<no parses (char 26):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : D s***  >>}}$ and if $ \ottnt{a}  \leadsto  \ottnt{a_{{\mathrm{1}}}} $, then $\texttt{\textcolor{red}{<<no parses (char 16):  \mbox{$\mid$}- D a ~>> D a1***  >>}}$; otherwise if $\ottnt{a}$ is a value, then so is $\texttt{\textcolor{red}{<<no parses (char 4):  D a***  >>}}$.
\end{theorem}

\begin{proof}
By induction on $\texttt{\textcolor{red}{<<no parses (char 11):  G \mbox{$\mid$}- a : s***  >>}}$.

\begin{itemize}
\item
For \rref{DCC-Var}, we have $\texttt{\textcolor{red}{<<no parses (char 29):  (G1 ++ x : s) ++ G2 \mbox{$\mid$}- x : s***  >>}}$. \\ We translate it to $     \overline{ \Gamma_{{\mathrm{1}}} }^{  { \color{black}{\bot} }  }  ,   \ottmv{x} \! :^{  { \color{black}{\bot} }  }\!  \overline{ \ottnt{s} }     ,   \overline{ \Gamma_{{\mathrm{2}}} }^{  { \color{black}{\bot} }  }    \vdash\,  \ottmv{x}  \, :^{  { \color{black}{\bot} }  }  \,   \overline{ \ottnt{s} }  $.
\item
For \rref{DCC-Unit}, we have $ \Gamma  \vdash  \,  \ottkw{unit}  \, : \,  \ottkw{Unit} $. \\ We translate it to $\texttt{\textcolor{red}{<<no parses (char 36):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot N top unit : D Unit***  >>}}$. 
\item
For \rref{DCC-Lam}, we have $\texttt{\textcolor{red}{<<no parses (char 25):  G \mbox{$\mid$}- \mbox{$\backslash{}$} x : s. b : s -> t***  >>}}$ where $  \Gamma  ,   \ottmv{x}  :  \ottnt{s}    \vdash  \,  \ottnt{b}  \, : \,  \ottnt{t} $. \\ By the inductive hypothesis, we get $\texttt{\textcolor{red}{<<no parses (char 41):  D bot G ++ x : bot D s \mbox{$\mid$}\mbox{$\mid$}- bot D b : D t***  >>}}$. \\ Now, using \rref{SDC-Lam}, we have, $\texttt{\textcolor{red}{<<no parses (char 45):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot \mbox{$\backslash{}$} x : D s . D b : D s -> D t***  >>}}$. \\ By promotion and \rref{SDC-Return}, we get, $\texttt{\textcolor{red}{<<no parses (char 95):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot N (\# M (\# s -> t \#) \#) (\mbox{$\backslash{}$} x : D s . D b) : T (\# M (\# s -> t \#) \#) (D s -> D t)***  >>}}$.
\item
For \rref{DCC-App}, we have $ \Gamma  \vdash  \,   \ottnt{b}  \;  \ottnt{a}   \, : \,  \ottnt{t} $ where $\texttt{\textcolor{red}{<<no parses (char 16):  G \mbox{$\mid$}- b : s -> t***  >>}}$ and $\texttt{\textcolor{red}{<<no parses (char 11):  G \mbox{$\mid$}- a : s***  >>}}$. \\ By the inductive hypothesis, we get $\texttt{\textcolor{red}{<<no parses (char 59):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D b :  T (\# M (\# s -> t \#) \#) (D s -> D t)***  >>}}$ and $\texttt{\textcolor{red}{<<no parses (char 26):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : D s***  >>}}$. \\ Let $\ell = \texttt{\textcolor{red}{<<no parses (char 21):  (\# M (\# s -> t \#) \#)***  >>}}$. Using \rref{SDC-Bind}, we get $\texttt{\textcolor{red}{<<no parses (char 51):  D bot G \mbox{$\mid$}\mbox{$\mid$}- psi bind psi x = D b in x : D s -> D t***  >>}}$. \\ Using \rref{SDC-App}, we have, $\texttt{\textcolor{red}{<<no parses (char 50):  D bot G \mbox{$\mid$}\mbox{$\mid$}- psi (bind psi x = D b in x) D a : D t***  >>}}$. \\ Again, using \rref{SDC-Return}, $ \texttt{\textcolor{red}{<<no parses (char 65):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot N psi  ((bind psi x = D b in x) D a) : T psi D t***  >>}}$. \\ Now, $\texttt{\textcolor{red}{<<no parses (char 10):  T psi D t***  >>}} =  T^{ \ell }\;   T^{ \ell }\;  \ottnt{t'}  $. Then, $\texttt{\textcolor{red}{<<no parses (char 65):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot join (N psi ((bind psi x = D b in x) D a)) : D t***  >>}}$. \\ So $\texttt{\textcolor{red}{<<no parses (char 12):  D (\# b a \#)***  >>}} = \texttt{\textcolor{red}{<<no parses (char 43):  join (N psi ((bind psi x = D b in x) D a))***  >>}}$. \\ Now, $ \ottnt{b}  \;  \ottnt{a} $ can step in three ways:
\begin{itemize}
\item $ \ottnt{b}  \leadsto  \ottnt{b_{{\mathrm{1}}}} $. Then, $\texttt{\textcolor{red}{<<no parses (char 16):  \mbox{$\mid$}- D b ~>> D b1***  >>}}$. So $\texttt{\textcolor{red}{<<no parses (char 32):  \mbox{$\mid$}- D (\# b a \#) ~>> D (\# b1 a \#)***  >>}}$.
\item $\ottnt{b}$ is a value and $ \ottnt{a}  \leadsto  \ottnt{a_{{\mathrm{1}}}} $. Then, $\texttt{\textcolor{red}{<<no parses (char 4):  D b***  >>}}$ is a value and $\texttt{\textcolor{red}{<<no parses (char 16):  \mbox{$\mid$}- D a ~>> D a1***  >>}}$. So $\texttt{\textcolor{red}{<<no parses (char 32):  \mbox{$\mid$}- D (\# b a \#) ~>> D (\# b a1 \#)***  >>}}$.
\item $\ottnt{b}$ and $\ottnt{a}$ are values. In this case, $\ottnt{b} = \texttt{\textcolor{red}{<<no parses (char 13):  \mbox{$\backslash{}$} x : s . b1***  >>}}$. And $\texttt{\textcolor{red}{<<no parses (char 4):  D b***  >>}} = \texttt{\textcolor{red}{<<no parses (char 25):  N psi (\mbox{$\backslash{}$} x : D s . D b1)***  >>}}$. 
\end{itemize}
\item
For \rref{DCC-Pair}, we have $\texttt{\textcolor{red}{<<no parses (char 25):  G \mbox{$\mid$}- (a , b) : s times t***  >>}}$ where $\texttt{\textcolor{red}{<<no parses (char 11):  G \mbox{$\mid$}- a : s***  >>}}$ and $ \Gamma  \vdash  \,  \ottnt{b}  \, : \,  \ottnt{t} $. \\ By the inductive hypothesis, $\texttt{\textcolor{red}{<<no parses (char 26):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : D s***  >>}}$ and $\texttt{\textcolor{red}{<<no parses (char 26):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D b : D t***  >>}}$. \\ By \rref{SDC-Pair}, we get $\texttt{\textcolor{red}{<<no parses (char 44):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot (D a , D b) : D s times D t***  >>}}$. \\ By promotion and \rref{SDC-Return}, $\texttt{\textcolor{red}{<<no parses (char 98):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot N (\# M (\# s times t \#) \#) (D a , D b) : T (\# M (\# s times t \#) \#) (D s times D t)***  >>}}$. \\ Since $\texttt{\textcolor{red}{<<no parses (char 10):  [\mbox{$\mid$} D a \mbox{$\mid$}]***  >>}} =  \llbracket  \ottnt{a}  \rrbracket $ and $\texttt{\textcolor{red}{<<no parses (char 10):  [\mbox{$\mid$} D b \mbox{$\mid$}]***  >>}} =  \llbracket  \ottnt{b}  \rrbracket $, so $ \texttt{\textcolor{red}{<<no parses (char 44):  [\mbox{$\mid$} N (\# M (\# s times t \#) \#) (D a , D b) \mbox{$\mid$}]***  >>}} =  \llbracket   ( \ottnt{a}  ,  \ottnt{b} )   \rrbracket $.
\item
For \rref{DCC-ProjF}, we have $\texttt{\textcolor{red}{<<no parses (char 15):  G \mbox{$\mid$}- fst a : s***  >>}}$ where $\texttt{\textcolor{red}{<<no parses (char 19):  G \mbox{$\mid$}- a : s times t***  >>}}$. \\ By the inductive hypothesis, $\texttt{\textcolor{red}{<<no parses (char 64):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : T (\# M (\# s times t \#) \#) (D s times D t)***  >>}}$. \\ Let $\ell = \texttt{\textcolor{red}{<<no parses (char 24):  (\# M (\# s times t \#) \#)***  >>}}$. Then, using \rref{SDC-Bind}, we get $\texttt{\textcolor{red}{<<no parses (char 54):  D bot G \mbox{$\mid$}\mbox{$\mid$}- psi bind psi x = D a in x : D s times D t***  >>}}$. \\ By \rref{SDC-ProjF}, $\texttt{\textcolor{red}{<<no parses (char 50):  D bot G \mbox{$\mid$}\mbox{$\mid$}- psi fst (bind psi x = D a in x) : D s***  >>}}$. \\ Now, since $\ell  \leq   \lceil  \ottnt{s}  \rceil $, by promotion $\texttt{\textcolor{red}{<<no parses (char 56):  D bot G \mbox{$\mid$}\mbox{$\mid$}- (\# M s \#) fst (bind psi x = D a in x) : D s***  >>}}$. \\ By \rref{SDC-Return}, $\texttt{\textcolor{red}{<<no parses (char 76):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot N (\# M s \#) (fst (bind psi x = D a in x)) : T (\# M s \#) D s***  >>}}$. \\ But $ \overline{ \ottnt{s} }  = \texttt{\textcolor{red}{<<no parses (char 15):  T (\# M s \#) s'***  >>}}$. So $\texttt{\textcolor{red}{<<no parses (char 71):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot join (N (\# M s \#) (fst (bind psi x = D a in x))) : D s***  >>}}$. \\ Then, $\texttt{\textcolor{red}{<<no parses (char 14):  D (\# fst a \#)***  >>}} = \texttt{\textcolor{red}{<<no parses (char 49):  join (N (\# M s \#) (fst (bind psi x = D a in x)))***  >>}}$. \\ Using the inductive hypothesis and lemma \ref{join}, we see that $ \pi_1\  \ottnt{a} $ and $\texttt{\textcolor{red}{<<no parses (char 14):  D (\# fst a \#)***  >>}}$ have the same meaning. \\ The \rref{DCC-ProjS} follows similarly.
\item 
For \rref{DCC-InjF}, we have $\texttt{\textcolor{red}{<<no parses (char 20):  G \mbox{$\mid$}- inj1 a : s + t***  >>}}$ where $\texttt{\textcolor{red}{<<no parses (char 11):  G \mbox{$\mid$}- a : s***  >>}}$. \\
By the inductive hypothesis, $\texttt{\textcolor{red}{<<no parses (char 26):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : D s*** >>}}$.\\
By \rref{SDC-InjF}, we have, $\texttt{\textcolor{red}{<<no parses (char 37):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot inj1 D a : D s + D t***  >>}}$.\\
By \rref{SDC-Return}, we get, $\texttt{\textcolor{red}{<<no parses (char 69):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot N bot (inj1 D a) : T (\# M (\# s + t \#) \#) (D s + D t)***  >>}}$. \\
Then, $\texttt{\textcolor{red}{<<no parses (char 15):  D (\# inj1 a \#)***  >>}} = \texttt{\textcolor{red}{<<no parses (char 17):  N bot (inj1 D a)***  >>}}$. By inductive hypothesis, $\texttt{\textcolor{red}{<<no parses (char 21):  [\mbox{$\mid$} D (\# inj1 a \#) \mbox{$\mid$}]***  >>}} =  \llbracket   \ottkw{inj}_1\,  \ottnt{a}   \rrbracket $.\\ 
The \rref{DCC-InjS} follows similarly.
\item
For \rref{DCC-Case}, we have $ \Gamma  \vdash  \,   \ottkw{case} \,  \ottnt{a} \, \ottkw{of}\,  \ottnt{b_{{\mathrm{1}}}}  ;  \ottnt{b_{{\mathrm{2}}}}   \, : \,  \ottnt{t} $ where $\texttt{\textcolor{red}{<<no parses (char 17):  G \mbox{$\mid$}- a : s1 + s2***  >>}}$ and $\texttt{\textcolor{red}{<<no parses (char 18):  G \mbox{$\mid$}- b1 : s1 -> t***   >>}}$ and $\texttt{\textcolor{red}{<<no parses (char 18):  G \mbox{$\mid$}- b2 : s2 -> t***  >>}}$. \\
By the inductive hypothesis, $\texttt{\textcolor{red}{<<no parses (char 42):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : T bot (D s1 + D s2)***  >>}}$ and $\texttt{\textcolor{red}{<<no parses (char 49):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D b1 : T (\# M t \#) (D s1 -> D t)***  >>}}$ and $\texttt{\textcolor{red}{<<no parses (char 49):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D b2 : T (\# M t \#) (D s2 -> D t)***  >>}}$. \\
By \rref{SDC-Bind}, we get, $\texttt{\textcolor{red}{<<no parses (char 19):  D bot G \mbox{$\mid$}\mbox{$\mid$}- (\# M t*** \#) bind x = D b1 in x : D s1 -> D t  >>}}$. \\
By \rref{SDC-Bind}, we get, $\texttt{\textcolor{red}{<<no parses (char 19):  D bot G \mbox{$\mid$}\mbox{$\mid$}- (\# M t*** \#) bind y = D b2 in x : D s2 -> D t  >>}}$. \\
By \rref{SDC-Case}, we get, $\texttt{\textcolor{red}{<<no parses (char 19):  D bot G \mbox{$\mid$}\mbox{$\mid$}- (\# M t*** \#) case D a of (bind x = D b1 in x); (bind y = D b2 in y) : D t  >>}}$. \\
By \rref{SDC-Return}, we get, $\texttt{\textcolor{red}{<<no parses (char 91):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot N (\# M t \#) (case D a of (bind x = D b1 in x); (bind y = D b2 in y)) : D t***  >>}}$. \\
By lemma \ref{join}, we have, $\texttt{\textcolor{red}{<<no parses (char 98):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot join (N (\# M t \#) (case D a of (bind x = D b1 in x); (bind y = D b2 in y))) : D t***  >>}}$. \\
Then, $\texttt{\textcolor{red}{<<no parses (char 25):  D (\# case a of b1; b2 \#)***  >>}} = \texttt{\textcolor{red}{<<no parses (char 76):  join (N (\# M t \#) (case D a of (bind x = D b1 in x); (bind y = D b2 in y)))***  >>}}$. \\
By inductive hypothesis and lemma \ref{join}, $\texttt{\textcolor{red}{<<no parses (char 31):  [\mbox{$\mid$} D (\# case a of b1; b2 \#) \mbox{$\mid$}]***  >>}} =  \llbracket   \ottkw{case} \,  \ottnt{a} \, \ottkw{of}\,  \ottnt{b_{{\mathrm{1}}}}  ;  \ottnt{b_{{\mathrm{2}}}}   \rrbracket $.
\item
For \rref{DCC-Return}, we have $\texttt{\textcolor{red}{<<no parses (char 23):  G \mbox{$\mid$}- N psi a : T psi s***  >>}}$ where $\texttt{\textcolor{red}{<<no parses (char 11):  G \mbox{$\mid$}- a : s***  >>}}$. \\
By inductive hypothesis, $\texttt{\textcolor{red}{<<no parses (char 26):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : D s***  >>}}$. \\
By promotion and \rref{SDC-Return}, we get, $\texttt{\textcolor{red}{<<no parses (char 76):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot N (\# psi \mbox{$\backslash{}$}/ M s \#) N psi D a : T (\# psi \mbox{$\backslash{}$}/ M s \#) T psi D s***  >>}}$. \\
Then, $\texttt{\textcolor{red}{<<no parses (char 16):  D (\# N psi a \#)***  >>}} = \texttt{\textcolor{red}{<<no parses (char 29):  N (\# psi \mbox{$\backslash{}$}/ M s \#) N psi D a***  >>}}$. \\
By inductive hypothesis, $\texttt{\textcolor{red}{<<no parses (char 22):  [\mbox{$\mid$} D (\# N psi a \#) \mbox{$\mid$}]***  >>}} =  \llbracket   \eta^{ \ell }\;  \ottnt{a}   \rrbracket $.
\item
For \rref{DCC-Bind}, we have $ \Gamma  \vdash  \,   \ottkw{bind}  \,  \ottmv{x}  =  \ottnt{a}  \,  \ottkw{in}  \,  \ottnt{b}   \, : \,  \ottnt{t} $ where $\texttt{\textcolor{red}{<<no parses (char 17):  G \mbox{$\mid$}- a : T psi s***  >>}}$ and $  \Gamma  ,   \ottmv{x}  :  \ottnt{s}    \vdash  \,  \ottnt{b}  \, : \,  \ottnt{t} $ and $ \ell  \leq  \ottnt{t} $.\\
By inductive hypothesis, $\texttt{\textcolor{red}{<<no parses (char 51):  D bot G \mbox{$\mid$}\mbox{$\mid$}- bot D a : T (\# psi \mbox{$\backslash{}$}/ M s \#) T psi D s***  >>}}$ and $\texttt{\textcolor{red}{<<no parses (char 41):  D bot G ++ x : bot D s \mbox{$\mid$}\mbox{$\mid$}- bot D b : D t***  >>}}$. 
\end{itemize}
\end{proof}

==> Sections/Section4.tex <==
\section{A Dependent Qualitiative Type System}

In this section we extend the simple system to include dependent types. 

First, some notation. We write $\phi < \ell$ when we have
$ \neg  \ottsym{(}  \ell  \leq  \phi  \ottsym{)} $ and $\phi  \leq  \ell$.

Dependent types provide both opportunities and difficulties. On one hand,
having a builtin notion of dependence is important in order to support
compile-time irrelevance: we would like to use the guarded version of
definitional equality in the conversion rule so that compile-time equivalence
can ignore parts of the term (as long as it is sound to do so).

\[ \drule{T-Conv} \] 

Which parts of terms should be ignored during conversion? As much as
possible. Because I don't yet know what that level should be, I'm going to
mark it as $\texttt{\textcolor{red}{<<no parses (char 8): type psi*** >>}}$ for now.

If this level is $ \top $, then we do not have any compile-time irrelevance.

If this level is $ \bot $, then we have as much compile-time irrelevance as possible.


\begin{itemize}

\item Type annotations in the term should be equated with a grade that is
  higher than all runtime grades. We do not annotate the argument types of
  lambda, but if we did, those argument types should allow both runtime and
  compile-time irrelevance.

\item If a variable \emph{only} appears in a type then it should be graded
  with a higher grade.

For example, consider a derivation for the polymorphic identity function. 

\[
   \varnothing  \vdash_{ \phi }   \lambda^{ \ell }  \ottmv{x}  .   \lambda^{ \phi }  \ottmv{y}  .  \ottmv{y}   : \ottsym{(}   \Pi  \ottmv{x} \!:^{ \ell }\!  \textbf{Type}  .  \Pi  \ottmv{y} \!:^{ \phi }\! \ottmv{x} . \ottmv{x}    \ottsym{)} 
\]

This means that we want to allow uses of this expression to mark arguments as
ignorable.

\[ 
   \varnothing  \vdash_{ \phi }   \ottsym{(}   \lambda^{ \ell }  \ottmv{x}  .   \lambda^{ \phi }  \ottmv{y}  .  \ottmv{y}    \ottsym{)}  \;  \ottkw{Unit} ^{ \ell }  :  {}^{ \phi } \!  \ottkw{Unit}  \to  \ottkw{Unit}  
\] 

If we have $ \neg  \ottsym{(}  \ell  \leq  \phi  \ottsym{)} $, then definitional equality gives us:

\[ 
   \varnothing  \vdash_{ \phi }   \ottsym{(}   \lambda^{ \ell }  \ottmv{x}  .   \lambda^{ \phi }  \ottmv{y}  .  \ottmv{y}    \ottsym{)}  \;  \ottkw{Unit} ^{ \ell }   \equiv   \ottsym{(}   \lambda^{ \ell }  \ottmv{x}  .   \lambda^{ \phi }  \ottmv{y}  .  \ottmv{y}    \ottsym{)}  \;  \ottkw{Bool} ^{ \ell }  
\] 

(Definitional equality is untyped, so these two expressions can be equated even though they have different types. There are longer examples that demonstrate the same idea, but equate terms with the same types.)

\item In functions, the use of the argument in the term (can be) different from its use in a type. 

  Going back to the previous example of the polymorphic identity function,
  notice that in the derivation, the variable $\ottmv{x}$ does not appear in the
  term but does appear in the type. This means that our typing rule for $\Pi$
  types needs to allow this different usage if we are to admit this example.


\[ \drule{T-Pi} \]

In otherwords, we cannot use $\ell_{{\mathrm{1}}}$ when we check $\ottnt{B}$, we need to use some other label $\ell_{{\mathrm{0}}}$, that is potentially $\ell_{{\mathrm{0}}}  \leq  \ell_{{\mathrm{1}}}$.

It does not seem likely that we will need to have $\ell_{{\mathrm{0}}}$ that is not $ \leq $ $\ell_{{\mathrm{1}}}$. 

\item We want to keep the formation rule for $\Pi$ types general and not fix it at a certain level. That will allow us to compare types at different levels. i.e. it might be the case that two types are equal at level $ { \color{red}{C} }  <  \top $

$ \varnothing  \vdash_{  { \color{red}{C} }  }   \Pi  \ottmv{x} \!:^{ \phi }\! \ottnt{A_{{\mathrm{1}}}} . \ottnt{B_{{\mathrm{1}}}}   \equiv   \Pi  \ottmv{x} \!:^{ \phi }\! \ottnt{A_{{\mathrm{2}}}} . \ottnt{B_{{\mathrm{2}}}}  $

where $ \top $-marked subterms inside the types can be ignored, but not equal at $ \top $.


\item Our ``regularity'' lemma for the type system must check types with 
  a ``higher'' grade.

  $ \Omega  \vdash_{ \phi }  \ottnt{a} : \ottnt{A} $ implies $ \Omega  \vdash_{ \ell }  \ottnt{A} :  \textbf{Type}  $

where $ \neg  \ottsym{(}  \ell  \leq  \phi  \ottsym{)} $. Furthermore, we'd also like to allow term variables to appear in types (this is the heart of dependent types) so we also need $\phi  \leq  \ell$.


If we are going to allow runtime irrelevance, we need to make sure that the $\ell$ we use to check types describes arguments that are not needed at runtime and allows them to be used in types.


\item But now consider the application rule: we need to use the argument in two places, in the term and in in the type.
We substitute in the type when type checking and in the body of the function during evaluation. Both of these substitutions must be good.

\[ \drule{T-App} \]

For the reasons described in the previous section, we need to check the argument using $ \ell_{{\mathrm{0}}}  \vee  \ell $.

But if we are going to show that $ \Omega  \vdash_{ \phi }  \ottnt{B}  \ottsym{\{}  \ottnt{a}  \ottsym{/}  \ottmv{x}  \ottsym{\}} :  \textbf{Type}  $ then we need to know that this argument is valid for the body of the $\Pi$ type.

\item Making the grade in the body of the pi the same as the grade on the lambda does NOT solve the issue with preservation. 

Going this route requires adding an assumption that the $\Pi$ is well formed in the abs rule because the level 
influences how types are checked.

\[ 
\frac{
  \Omega ,   \ottmv{x} \! :^{  \ell_{{\mathrm{0}}}  \vee  \ell  }\! \ottnt{A}    \vdash_{ \ell }  \ottnt{b} : \ottnt{B}  \qquad
\texttt{\textcolor{red}{<<no parses (char 8): W \mbox{$\mid$}-- ty***pe psi (Pi x:psi0 A. B) : type >>}}
}{
 \Omega  \vdash_{ \ell }   \lambda^{ \ell_{{\mathrm{0}}} }  \ottmv{x}  .  \ottnt{b}  :  \Pi  \ottmv{x} \!:^{ \ell_{{\mathrm{0}}} }\! \ottnt{A} . \ottnt{B}  
}
\]

This modification is enough for regularity. But not for preservation.
The problem is that if definitional equality is at some fixed level $ { \color{red}{C} } $, we have the argument 
graded at $\texttt{\textcolor{red}{<<no parses (char 6): psi0 **** psi >>}}$. But we need it to be graded at $\texttt{\textcolor{red}{<<no parses (char 6): psi0 **** CTime >>}}$. As in the prior version, 
we don't know whether $\ell  \leq   { \color{red}{C} } $>


\end{itemize}




